Reflexive polygons and rational elliptic surfaces

In this note we study in detail the geometry of eight rational elliptic surfaces naturally associated to the sixteen reflexive polygons. The elliptic fibrations supported by these surfaces correspond under mirror symmetry to the eight families of smooth del Pezzo surfaces with very ample anticanonical bundle.

==> Commands.tex <==
%general symbols
\renewcommand{\setminus}{\smallsetminus}
\renewcommand{\emptyset}{\varnothing}
\newcommand{\epsi}{\varepsilon}
\newcommand{\phiv}{\varphi}
%\newcommand{\epsi}{\varepsilon}
%\newcommand{\inv}{^{-1}}
\newcommand{\into}{\hookrightarrow} %monomorfismo
\newcommand{\onto}{\twoheadrightarrow} %epimorfismo
\newcommand{\id}{\mathrm{id}} %identita`
%\def\der#1#2{\frac{\partial #1}{\partial #2}} %derivata parziale
\newcommand{\GL}{\mathrm{GL}} %general linear group
\newcommand{\SL}{\mathrm{SL}} %general linear group
%\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\rank}{rank}
%\DeclareMathOperator{\embdim}{embdim}
\newcommand{\Gm}{\mathbb{G}_\mathrm{m}}
\newcommand{\al}{\alpha}
\newcommand{\chitop}{\chi_\mathrm{top}}
\newcommand{\contr}{\mathrm{contr}}
\newcommand{\tors}{\mathrm{tors}}
\newcommand{\trop}{\mathrm{trop}}

\newcommand{\bfone}{\boldsymbol{1}}
\DeclareMathOperator{\Vol}{Vol}
\newcommand{\pencilP}{\mathfrak{d}_P}
\newcommand{\minresYP}{\overline{Y}_{P}}
\newcommand{\barDP}{\overline{D}_{P}}

%general algebraic geometry symbols
%\DeclareMathOperator\Aut{Aut}
%\DeclareMathOperator{\Sing}{Sing}
%\DeclareMathOperator{\spe}{sp}
\DeclareMathOperator{\Hom}{Hom} %spazio degli omomorfismi
%\DeclareMathOperator{\RHom}{RHom} %spazio degli omomorfismi
\newcommand{\Ext}{\mathrm{Ext}}
\newcommand{\cExt}{\mathcal{E}xt}
\newcommand{\cHom}{\mathcal{H}om}
%\newcommand{\SSpec}{\mathbf{Spec}}
%\newcommand{\cSym}{\mathcal{S}ym}
\DeclareMathOperator{\Spec}{Spec} %spettro di un anello
\DeclareMathOperator{\Proj}{Proj} %spazio proiettivo
\DeclareMathOperator{\Pic}{Pic}
\DeclareMathOperator{\Cl}{Cl}

\DeclareMathOperator{\MW}{MW} %Mordell-Weil lattice
\DeclareMathOperator{\NS}{NS} 

\newcommand{\Newt}[1]{\mathrm{Newt}(#1)}

\newcommand{\bmu}{\boldsymbol{\mu}}

%\def\HilbS#1{\mathrm{Hilb}( #1 , -K_{#1})}
\newcommand{\pow}[1]{[ \!  [ #1 ] \! ]}

%\def\pow#1{ \llbracket  #1 \rrbracket }



%Fano
\newcommand{\morimukai}[2]{$\mathrm{MM}_{#1 - #2}$} %mori-mukai list
%\newcommand{\delpezzo}{\mathrm{dP}}

%K-moduli
\newcommand{\Kss}[2]{ \mathcal{M}^\mathrm{Kss}_{#1, #2} } %K-moduli stack
\newcommand{\Kps}[2]{M^\mathrm{Kps}_{#1, #2}} %K-moduli space

%\newcommand{\coh}[2]{\mathrm{H}^{#1}(#2, \mathbb{Q})} %cohomology


%Deformations
%\newcommand{\art}{(\mathrm{Art}_{\Bbbk})}
%\newcommand{\comp}{(\mathrm{Comp}_{\Bbbk})}
%\newcommand{\compC}{(\mathrm{Comp}_\mathbb{C})}
%\newcommand{\set}{(\mathrm{Set})}

%\DeclareMathOperator{\Spf}{Spf}
%\newcommand{\Def}[1]{\mathrm{Def}_{#1}}
%\newcommand{\Defloc}[1]{\mathrm{Def}^\mathrm{loc}_{#1}}
%\newcommand{\loc}{\mathrm{loc}}
%\newcommand{\ob}{\mathrm{ob}}




%groupoids
%\newcommand{\grpd}{(\mathrm{Grpd})}
%\newcommand{\gDef}[1]{\mathcal{D}ef_{#1}}

%derived
%\newcommand{\dart}{(\mathrm{SArt}_k)}
%\newcommand{\dDef}[1]{\mathbf{Def}_{#1}}
%\newcommand{\spaces}{\mathscr{S}}
%\newcommand{\underive}[1]{\vert #1 \vert}

%qGorenstein
\newcommand{\DefqG}[1]{\mathrm{Def}^{\mathrm{qG}}_{#1}}
\newcommand{\TTqG}[2]{\mathbb{T}^{\mathrm{qG}, #1}_{#2}}
\newcommand{\cTqG}[2]{\mathscr{T}^{\mathrm{qG}, #1}_{#2}}
\newcommand{\Def}[1]{\mathrm{Def}_{#1}}


%discrete geometry symbols
%\def\conv#1{\mathrm{conv} \left\{ #1  \right\} } %convex hull
%\DeclareMathOperator{\Span}{Span} %sottosp vettoriale generato
%\def\spanR#1{\mathrm{span}_\mathbb{R} \left( #1 \right)} 
%\newcommand{\vertices}{\mathrm{vert}} %vertices of a polyhedron
%\newcommand{\cone}{\mathrm{cone}}
%\def\cone#1{\mathrm{cone} \left\{ #1 \right\}}



%%%%%%%%%%%%%%%%%%%%%%%

%alphabets

%calligrafico maiuscolo
\newcommand\cB{\mathcal{B}}
\newcommand\cD{\mathcal{D}}
\newcommand\cE{\mathcal{E}}
\newcommand\cF{\mathcal{F}}
\newcommand\cG{\mathcal{G}}
\newcommand\cH{\mathcal{H}}
\newcommand\cI{\mathcal{I}}
\newcommand\cL{\mathcal{L}}
\newcommand\cM{\mathcal{M}}
\newcommand\cO{\mathcal{O}}
\newcommand\cR{\mathcal{R}}
\newcommand\cS{\mathcal{S}}
\newcommand\cX{\mathscr{X}}
\newcommand\cU{\mathcal{U}}
\newcommand\cV{\mathcal{V}}


%veramente calligrafico
\newcommand\cT{\mathscr{T}}
%\newcommand\scrX{\mathscr{X}}
%\newcommand\scrY{\mathscr{Y}}
%\newcommand\scrZ{\mathscr{Z}}

%grassetto matematico maiuscolo
\renewcommand\AA{\mathbb{A}}
\newcommand\CC{\mathbb{C}}
\newcommand\FF{\mathbb{F}}
\newcommand\GG{\mathbb{G}}
%\newcommand{\KK}{\mathbb{K}}
\newcommand{\KK}{\Bbbk}
\newcommand{\LL}{\mathbb{L}}
\newcommand\NN{\mathbb{N}}
\newcommand\PP{\mathbb{P}}
\newcommand\QQ{\mathbb{Q}}
\newcommand\RR{\mathbb{R}}
\newcommand\TT{\mathbb{T}}
\newcommand\ZZ{\mathbb{Z}}

%dritto maiuscolo
\newcommand\rG{\mathrm{G}}
\newcommand\rH{\mathrm{H}}
\newcommand\rL{\mathrm{L}}
\newcommand\rR{\mathrm{R}}
\newcommand{\rT}{\mathrm{T}}
\newcommand\rV{\mathrm{V}}

%dritto minuscolo
\newcommand\rmm{\mathrm{m}}
\newcommand\rmd{\mathrm{d}}

%gotico minuscolo
\newcommand{\frakm}{\mathfrak{m}}
\newcommand{\frakp}{\mathfrak{p}}

%gotico maiuscolo
\newcommand{\frakX}{\mathfrak{X}}
\newcommand{\frakY}{\mathfrak{Y}}

